kNet: A Deep kNN Network To Handle Label Noise

Deep Neural Networks require large amounts of labeled data for their training. Collecting this data at scale inevitably causes label noise.Hence,the need to develop learning algorithms that are robust to label noise. In recent years, k Nearest Neighbors (kNN) emerged as a viable solution to this problem. Despite its success, kNN is not without its problems. Mainly, it requires a huge memory footprint to store all the training samples and it needs an advanced data structure to allow for fast retrieval of the relevant examples, given a query sample. We propose a neural network, termed kNet, that learns to perform kNN. Once trained, we no longer need to store the training data, and processing a query sample is a simple matter of inference. To use kNet, we first train a preliminary network on the data set, and then train kNet on the penultimate layer of the preliminary network.We find that kNet gives a smooth approximation of kNN,and cannot handle the sharp label changes between samples that kNN can exhibit. This indicates that currently kNet is best suited to approximate kNN with a fairly large k. Experiments on two data sets show that this is the regime in which kNN works best,and can therefore be replaced by kNet.In practice, kNet consistently improve the results of all preliminary networks, in all label noise regimes, by up to 3%.

==> backup_04_results.tex <==
\section{Experiments}

We evaluated our algorithm on the cifar-10 and SVHN datasets.


\subsection{Cifar10 and SVHN}

Next, we test the performance of the deep knn on bigger and realistic dataset such as Cifar10 and SVHN.
We added a 30\% asymmetric noise ratio \shai{What is asymmetric noise?}, and trained an end-to-end Resnet 20 which has 0.27M parameters. Next we trained a deep knn network on the penultimate layer and summarize the results of the different chosen $k$ in table 123.



\subsection{End-To-End Training With Noise Labels}

Next, we test the performance of the deep knn on bigger and realistic dataset such as Cifar10 and SVHN.
We added a 30\% asymmetric noise ratio, and trained an end-to-end resnet 20 which has 0.27M parameters.
Next we trained a deep knn network on the second to the last layer and summarize the results of the different chosen k (see tables 123, 234.

\begin{table}
\begin{center}
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
Network & Parameters & \multicolumn{5}{c}{ K } \\ \hline
& & 1 & 11 & 41 & 61 & 101 \\ \hline
Resnet20 & 0.27M & \multicolumn{5}{c}{ 75.28 } \\ \hline
Resnet20 + Knn & 0.27M + 3.2M & 61.49 & 85.51 & 87.84 & 87.74 & 87.56 \\ \hline
Resnet20 + DeepKnn & 0.27M + 3K & 87.49 & 87.53 & 87.43 & 87.38 & 87.38 \\ \hline
Resnet20 + FixedDeepKnn & 0.27M + 3K & 88.01 & \textbf{88.23} & 87.9 & 87.84 & 87.82 \\ \hline
\end{tabular}
\end{center}
\caption{Cifar10 - $30\%$ asymmetric noise}
\label{tab:cifar10-30}
\end{table}

\begin{table}
\begin{center}
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Network & Parameters & \multicolumn{4}{c}{ K } \\ \hline
& & 1 & 21 & 61 & 101 \\ \hline
Resnet20 & 0.55M & \multicolumn{4}{c}{ 58.02 } \\ \hline
Resnet20 + Knn & 0.55M+37.5M & 56.61 & 58.53 & 58.48 & 58.42 \\ \hline
Resnet20 + DeepKnn & 0.55M+4K & 58.32 & 58.33 & 58.33 & 58.32 \\ \hline
Zhang {\em et al.} \cite{Zhang20} & 0.87M & \multicolumn{4}{c}{ 91.88 } \\ \hline
Zhang {\em et al.} \cite{Zhang20} + Knn & 0.87M + 12.8M & 90.14 & \textbf{93.39} & 93.2 & 93.07 \\ \hline
Zhang {\em et al.} \cite{Zhang20} + DeepKnn & 0.87M + 5K & 93.09 & 93.07 & 93.11 & 93.08 \\ \hline
Zhang {\em et al.} \cite{Zhang20} + FixedDeepKnn & 0.87M + 5K & 92.88 & 92.9 & 92.81 & 92.73 \\ \hline
\end{tabular}
\end{center}
\caption{SVHN - 40\% symmetric noise}
\label{tab:SVHN-40}
\end{table}

\begin{table}
\begin{center}
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Network & Parameters & \multicolumn{4}{c}{ K } \\ \hline
& & 1 & 11 & 41 & 101 \\ \hline
Zhang {\em et al.} \cite{Zhang20} & 0.87M & \multicolumn{4}{c}{ 89.26 } \\ \hline
Zhang {\em et al.} \cite{Zhang20}+ Knn & 0.87M + 12.8M & 88.28 & 91.69 & 91.7 & 91.61 \\ \hline
Zhang {\em et al.} \cite{Zhang20}+ DeepKnn & 0.87M + 5K & 91.34 & 91.46 & 91.57 & 91.3068531 \\ \hline
Zhang {\em et al.} \cite{Zhang20} + FixedDeepKnn & 0.87M + 5K & 91.43 & \textbf{91.81} & 91.42 & 91.09 \\ \hline
\end{tabular}
\end{center}
\caption{SVHN - 80\% symmetric noise}
\label{tab:SVHN-80}
\end{table}


\subsection{Model Enhancement}

Zhang et al, presented a holistic framework to train deep neural networks in a way that is highly invulnerable to label
noise.
Taking it to the next step - we trained their network and apply KNN and DeepKnn to the second to the last layer.
Adding the DeepKnn network enhanced the network performance as shown in tables 4 and table 5.


\begin{table}
\begin{center}
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Network & Parameters & \multicolumn{4}{c}{ K } \\ \hline
& & 1 & 11 & 51 & 101 \\ \hline
Zhang {\em et al.} \cite{Zhang20} & 0.87M & \multicolumn{4}{c}{ 84.87 } \\ \hline
Zhang {\em et al.} \cite{Zhang20} + Knn & 0.87M + 12.8M & 82.41 & 86.11 & \textbf{86.16} & 85.85 \\ \hline
Zhang {\em et al.} \cite{Zhang20} + DeepKnn & 0.87M + 5K & 84.81 & 85.35 & 85.5 & 85.25 \\ \hline
Zhang {\em et al.} \cite{Zhang20} + FixedDeepKnn & 0.87M + 5K & 85.99 & 85.89 & 85.38 & 85.27 \\ \hline
\end{tabular}
\end{center}
\caption{Cifar10 - $80\%$ symmetric noise}
\label{tab:cifar10-80}
\end{table}

\begin{table}
\begin{center}
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Network & Parameters & \multicolumn{4}{c}{ K } \\ \hline
& & 1 & 11 & 51 & 101 \\ \hline
Resnet20 & 0.27M & \multicolumn{4}{c}{ 48.68 } \\ \hline
Resnet20+Knn & 0.27M + 5K & 27.44 & 41.57 & 48.66 & 49.09 \\ \hline
Resnet20+DeepKnn & 0.27M + 5K & 49.43 & 49.4 & 49.76 & 49.69 \\ \hline
Zhang {\em et al.} \cite{Zhang20} & 0.87M & \multicolumn{4}{c}{ 89.58 } \\ \hline
Zhang {\em et al.} \cite{Zhang20} + Knn & 0.87M + 12.8M & 86.92 & 89.56 & 89.42 & 89.27 \\ \hline
Zhang {\em et al.} \cite{Zhang20} + DeepKnn & 0.87M + 5K & 89.24 & 89.43 & 89.63 & 89.53 \\ \hline
Zhang {\em et al.} \cite{Zhang20} + FixedDeepKnn & 0.87M + 5K & \textbf{89.88} & 89.84 & 89.34 & 89.2 \\ \hline
\end{tabular}
\end{center}
\caption{Cifar10 - 40\% symmetric noise}
\label{tab:cifar10-40} 
\end{table}

\section{Model Enhancement}
    \begin{figure}
        \centering
        \includegraphics[scale=0.55]{cifar_dist_0_8_sad}
        \caption{Cifar-10, 80\% noise labels -  Dnn Vs Knn}
        \label{fig:my_label}
    \end{figure}
    \begin{figure}
        \centering
        \includegraphics[scale=0.55]{cifar_dist_0_4_sad}
        \caption{Zhang et al Cifar10 40\% noise labels - Dnn Vs Knn.\\ The upper graph represents the mean of absolute difference between the normalized kNN and the DkNN prediction along different k's.
        The lower graph represents the average maximum values of the the normalized kNN and the DkNN prediction.
        Although being trained on various k's, Our DkNN in is less sensitive to the selected k and is much more close to kNN with large k's.}
        \label{fig:my_label}
    \end{figure}
    






==> backup_tables.tex <==
\begin{table}
\begin{center}
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\multicolumn{6}{|c|}{ {\bf cifar-10} }\\
\hline
Network & Parameters & \multicolumn{4}{c|}{ K } \\ \hline
& & 1 & 11 & 61 & 101 \\ \hline
Resnet20 & 0.27M & \multicolumn{4}{c|}{ 75.28 } \\ \hline
~~~ + kNN & 0.27M + 3.2M & 61.49 & 85.51 & {\bf 87.74} & 87.56 \\ \hline
~~~ + kNet & 0.27M + 3K & 87.49 & {\bf 87.53} & 87.38 & 87.38 \\ \hline
Zhang {\em et al.}~\cite{Zhang20} & 0.87M & \multicolumn{4}{c|}{ 88.79 } \\ \hline
~~~ + kNN & 0.87M + 12.8M & 85.23 & 88.4 & {\bf 88.51} & 88.51 \\ \hline
~~~ + kNet & 0.87M + 5K & 88.63 & 88.84 & {\bf 88.89} & 88.35 \\ \hline
~~~ + fixed kNet & 0.87M + 5K & \textbf{88.94} & 88.88 & 88.91 & 88.87 \\ \hline
\multicolumn{6}{|c|}{ {\bf SVHN} }\\
\hline
Network & Parameters & \multicolumn{4}{c|}{ K } \\ \hline
& & 1 & 11 & 51 & 101 \\ \hline
CNN (CE loss) & 0.55M & \multicolumn{4}{c|}{ 88.23 } \\ \hline
~~~ + kNN & 0.55M+37.5M & 61.08 & 85.2 & 89.4 & {\bf 89.56} \\ \hline
~~~ + kNet & 0.55M+4K & 89.27 & 89.27 & {\bf 89.28} & 89.24 \\ \hline
Zhang {\em et al.}~\cite{Zhang20} & 0.87M & \multicolumn{4}{c|}{ 92.06 } \\ \hline
~~~ + kNN & 0.87M + 12.8M & 90.56 & {\bf 93.47} & 93.36 & 93.24 \\ \hline
~~~ + kNet & 0.87M + 5K & 92.36 & 92.71 & {\bf 93.02} & 92.88 \\ \hline
~~~ + fixedk Net & 0.87M + 5K & \textbf{93.4} & 93.04 & 93.12 & 93.07 \\ \hline

\end{tabular}
\end{center}
\caption{ {\bf ${\bf 30\%}$ random asymmetric label noise:} We show results on both cifar-10 (top) and SVHN (bottom) when adding $30\%$ of asymetric label noise. kNN, kNet, and fixed kNet run on the penultimate layer of different preliminary networks: ResnNet20, CNN, and Zhang {\em et al.}~\cite{Zhang20}. Best result in each row is marked in {\bf bold}. kNet and fixed kNet always improve the preliminary network. kNet requires $3k$ to $5k$ parameters, compared to $3.2M$ up to $12.8M$ parameters of kNN.}
\label{tab:asymetric_30}
\end{table}

\section{Experiments}

We evaluated our algorithm on the cifar-10 and SVHN datasets, using different preliminary network architectures and different noise models.

In all cases, kNN was applied to the penultimate layer where $k$ was randomly chosen in a range of $[1-101]$. kNN'm memory size composed by the size of the feature vector of the penultimate layer multiplied by the number of samples. In contrast, our kNet is a simple fully-connected based network with only one hidden state. The motivation of picking a small network was that we want a smooth and even underfit convergence in some noisy samples. 

\paragraph{Label noise}

We considered three noise models in the following experiments. In all cases, the noise was added by a transition matrix specifying the probability of one label being flipped to another. We corrupt the labels in the training data set for a fraction of the examples, the experiment’s “noise rate”,using one of three schemes::
\textbf{Uniform noise}: The label is flipped to any one of the labels (including itself) with equal probability (the transition matrix is symmetric across the classes)\\
\textbf{Semantic asymmetric noise}: A flipped label would be assign to 
 semantically-similar class \cite{DBLP:conf/cvpr/PatriniRMNQ17} (e.g., truck and automobile, or bird and airplane)\\
 \textbf{Random asymmetric noise}: A flipped label would be assign to one of two other random labels with probability of 66.6\% to one class and 33.3\% to the second.\\
 
\paragraph{fixed kNet} Our toy experiment and the work of \cite{DBLP:conf/icml/BahriJG20} demonstrate how kNet is stable and robust to the choice of $k$. While kNN's accuracy drops dramatically as $k$ gets lower, kNet performance might even get better.
For comparison, we added a fixed kNet experiment where instead of choosing $k$ at random during training, our kNet gets as an input a fixed $k$ in all iterations of training.
Surprisingly (mostly when k=1), the consistency and the performance of the kNet were maintained. In some of the fixed kNet experiments applying it with k=1 even gave the best accuracy.

% \begin{table}
% \begin{center}
% \scriptsize
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
% Network & Parameters & \multicolumn{4}{c|}{ K } \\ \hline
% & & 1 & 11 & 61 & 101 \\ \hline
% Resnet20 & 0.27M & \multicolumn{4}{c|}{ 75.28 } \\ \hline
% ~~~ + kNN & 0.27M + 3.2M & 61.49 & 85.51 & 87.74 & 87.56 \\ \hline
% ~~~ + kNet & 0.27M + 3K & 87.49 & 87.53 & 87.38 & 87.38 \\ \hline
% Zhang et al & 0.87M & \multicolumn{4}{c|}{ 88.79 } \\ \hline
% ~~~ + kNN & 0.87M + 12.8M & 85.23 & 88.4 & 88.51 & 88.51 \\ \hline
% ~~~ + kNet & 0.87M + 5K & 88.63 & 88.84 & 88.89 & 88.35 \\ \hline
% ~~~ + fixed kNet & 0.87M + 5K & \textbf{88.94} & 88.88 & 88.91 & 88.87 \\ \hline

% \end{tabular}
% \end{center}
% \caption{Cifar10 - $30\%$ random asymmetric noise}
% \label{tab:cifar10-30}
% \end{table}

% \begin{table}
% \begin{center}
% \scriptsize
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
% Network & Parameters & \multicolumn{4}{|c|}{ K } \\ \hline
% & & 1 & 11 & 51 & 101 \\ \hline
% CNN (CE loss) & 0.55M & \multicolumn{4}{|c|}{ 88.23 } \\ \hline
% ~~~ + kNN & 0.55M+37.5M & 61.08 & 85.2 & 89.4 & 89.56 \\ \hline
% ~~~ + kNet & 0.55M+4K & 89.27 & 89.27 & 89.28 & 89.24 \\ \hline
% Zhang et al & 0.87M & \multicolumn{4}{|c|}{ 92.06 } \\ \hline
% ~~~ + kNN & 0.87M + 12.8M & 90.56 & 93.47 & 93.36 & 93.24 \\ \hline
% ~~~ + kNet & 0.87M + 5K & 92.36 & 92.71 & 93.02 & 92.88 \\ \hline
% ~~~ + fixedk Net & 0.87M + 5K & \textbf{93.4} & 93.04 & 93.12 & 93.07 \\ \hline

% \end{tabular}
% \end{center}
% \caption{SVHN - $30\%$ random asymmetric noise}
% \label{tab:SVHN-30}
% \end{table}



\begin{figure*}[h!]
\begin{center}
\begin{tabular}{c c c}
\includegraphics[width=0.3\linewidth]{LaTeX/figures/ABC/ABC_0.3_pdf.png} &
\includegraphics[width=0.3\linewidth]{LaTeX/figures/Cifar/cifar10_res29_0.8_pdf.png} &
\includegraphics[width=0.3\linewidth]{LaTeX/figures/SVHN/svhn_res29_0.8_pdf.png} \\
\includegraphics[width=0.3\linewidth]{LaTeX/figures/ABC/ABC_0.3_sad.png} &
\includegraphics[width=0.3\linewidth]{LaTeX/figures/Cifar/cifar10_res29_0.8_vote.png} &
\includegraphics[width=0.3\linewidth]{LaTeX/figures/SVHN/svhn_res29_0.8_vote.png} \\
\end{tabular}\\
\caption{\textbf{kNet vs kNN}.The upper graphs represents the mean of absolute difference between the normalized kNN and the kNet prediction along different k's. The lower graph represents the average maximum values of the the normalized kNN and the kNet prediction. Although being trained on various k's, Our kNet in is less sensitive to the selected k and is much more close to kNN with large k's.}
\label{fig:dnn_kk}
\end{center}
\end{figure*}

\subsection{End-to-end training with noisy labels}

Motivated by the toy example, we started by adding a 30\% random asymmetric noise ratio to both cifar-10 and SVHN.
Each netwrok was trained from scartch, for cifar10 we used a Resnet20, while for SVHN training was done with a standard CNN \footnote{We follow \href{https://github.com/tohinz/SVHN-Classifier/blob/master/svhn_classifier.py}{this implementation} which contains 0.55M parameters}. For both of the experiments the training was done with a standard cross-entropy (CE) loss, without adding any noise-robust terms or cleaning data manipulation. Then, we applied kNN to the penultimate representation of the Resnet20 network and trained a kNet (where $k$ is part of the input during training) and kNet (where $k$ is fixed during training).

We performed this experiment for both cifar-10 and SVHN and report results in tables \ref{tab:cifar10-30} and \ref{tab:SVHN-30}. As can be seen, in both cases, all three kNN variants (kNN, kNet, and fixed kNet) improve the performance of the base Resnet20 network. In the case of cifar-10, the improvement is quite dramatic (from about $75\%$ to about $88\%$ in all three variants). 

On both data sets, kNN with $k=1$ performs much worst than the base Resnet20 network. Results improve dramatically as we increase $k$. The classification results for both kNet and fixed kNet are quite similar and consistent across the different $k$ values. This is to be expected because our network is quite small and offers a very smooth approximation of kNN, which corresponds to classification with a large $k$.

In addition, observe that the memory footprint of kNet and fixed kNet is just $3K$ or $4K$, compared to $3.2M$ and $37.5M$ for kNN, on cifar-10 and SVHN, respectively.


As can be seen in the toy example~\ref{fig:toy_example}, kNet tends to smooth out the results. This is further evident in the last experiment (Tables~\ref{tab:cifar10-30} and~\ref{tab:SVHN-30}) where the best performing kNet algorithm was for $k=51$ or $k=61$.
Intuitively, this suggests the kNet approximates kNN with a large $k$. 

To validate this assumption we have compared the probability distribution function (pdf) of kNN with the one produced by kNet, for different values of $k$. Results can be seen in Figure~\ref{fig:dnn_kk}. On top with see the absolute different between the pdd of kNet and that of kNN, for various $k$ values. As can be seen, there is a large gap at low $k$ values, and the minimum is achieved at around $50$ or $60$. This observation holds true for all data sets considered in this work.

Figure~\ref{fig:dnn_kk} (bottom) shows the maximum value in the pdf of both kNN and kNet. As can be seen, the maximum value is almost identical for both methods, except for $k=1$ where there is a large gap between the two. We conclude that kNet approximates kNN with a large $k$.


In the next experiment, we add $40\%$ uniform label noise and report the results for cifar-10 and SVHN in tables~\ref{tab:cifar10-40} and~\ref{tab:SVHN-40}, respectively. We see that Resnet20 behaves poorly in this experiment. Still, the three kNN variants improve it (except for the kNN with $k=1$ variant that fails miserably). 

A similar pattern can be observed when using the much stronger baseline network of Zhan {\em et al.} \cite{Zhang20}. They presented a holistic framework to train deep neural networks in a way that is highly invulnerable to label noise. Their approach , besides of re-weighting estimated  suspected noisy labels samples, combines an ongoing relabeling process based on pseudo labels that are  sharp and consistent across augmented versions of input. To the best of our knowledge, their paper is the first to demonstrate superior robustness against noise regimes as high as over $90\%$.
Yet, Zhang et al rely on a prior which is the presence of a small trusted data (i.e. probe data). In both of our experiments we set M, which indicates the number of trusted data used, to be M=0.01K. In our case it means 10 images per class.
Our kNN variants improve their performance by up to $2\%$ in the case of cifar-10 and $0.3\%$ in the SVHN case. In both cases, the kNet network requires a modest increase of $3K$ to $5K$ in memory.

We repeated this experiment with $80\%$ uniform noise and observed the same behaviour. A kNN variant improves the baseline network by about $2\%$ in both cifar-10 and SVHN. See Tables~\ref{tab:cifar10-80} and~\ref{tab:SVHN-80}.




\begin{table}
\begin{center}
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Network & Parameters & \multicolumn{4}{c}{ K } \\ \hline
& & 1 & 11 & 51 & 101 \\ \hline
Resnet20 (CE) & 0.27M & \multicolumn{4}{c}{ 66.43 } \\ \hline
~~~ + kNN & 0.27M + 5K & 38.95 & 62.01 & 65.72 & 66.92 \\ \hline
~~~ + kNet & 0.27M + 5K & 67.05 & 67.16 & 66.93 & 65.99 \\ \hline 
Zhang{\em et al.} \cite{Zhang20} & 0.87M & \multicolumn{4}{c}{ 89.58 } \\ \hline
~~~ + kNN & 0.87M + 12.8M & 86.92 & 89.56 & 89.42 & 89.27 \\ \hline
~~~ + kNet & 0.87M + 5K & 89.24 & 89.43 & 89.63 & 89.53 \\ \hline
~~~ + fixed kNet & 0.87M + 5K & \textbf{89.88} & 89.84 & 89.34 & 89.2 \\ \hline
\end{tabular}
\end{center}
\caption{Cifar10 - 40\% uniform noise}
\label{tab:cifar10-40} 
\end{table}

\begin{table}
\begin{center}
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Network & Parameters & \multicolumn{4}{c}{ K } \\ \hline
& & 1 & 21 & 61 & 101 \\ \hline
CNN (CE loss) & 0.55M & \multicolumn{4}{c}{ 92.92 } \\ \hline
~~~ + kNN & 0.55M+37.5M &  56.45 & 92.13 & 93.03 & 93.07  \\ \hline
~~~ + kNet & 0.55M+4K & 92.97 & 92.99 & 93.01 & 93.02 \\ \hline
Zhang {\em et al.} \cite{Zhang20} & 0.87M & \multicolumn{4}{c}{ 91.88 } \\ \hline
~~~ + kNN & 0.87M + 12.8M & 90.14 & \textbf{93.39} & 93.2 & 93.07 \\ \hline
~~~ + kNet & 0.87M + 5K & 93.09 & 93.07 & 93.11 & 93.08 \\ \hline
~~~ + fixedkNet & 0.87M + 5K & 92.88 & 92.9 & 92.81 & 92.73 \\ \hline
\end{tabular}
\end{center}
\caption{SVHN - 40\% uniform noise}
\label{tab:SVHN-40}
\end{table}


\begin{table}
\begin{center}
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Network & Parameters & \multicolumn{4}{|c|}{ K } \\ \hline
& & 1 & 11 & 51 & 101 \\ \hline
Resnet20 & 0.27M & \multicolumn{4}{|c|}{ 19.1 } \\ \hline
~~~ + kNN & 0.27M + 5K & 12.07 & 14.42 & 18.44 & 20.86 \\ \hline
~~~ + kNet & 0.27M + 5K & 24.56 & 24.99 & 25.9 & 26.18 \\ \hline
Zhang {\em et al.} \cite{Zhang20} & 0.87M & \multicolumn{4}{c}{ 84.87 } \\ \hline
~~~ + kNN & 0.87M + 12.8M & 82.41 & 86.11 & \textbf{86.16} & 85.85 \\ \hline
~~~ + kNet & 0.87M + 5K & 84.81 & 85.35 & 85.5 & 85.25 \\ \hline
~~~ + fixed kNet & 0.87M + 5K & 85.99 & 85.89 & 85.38 & 85.27 \\ \hline
\end{tabular}
\end{center}
\caption{Cifar10 - $80\%$ uniform noise}
\label{tab:cifar10-80}
\end{table}



\begin{table}
\begin{center}
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Network & Parameters & \multicolumn{4}{|c|}{ K } \\ \hline
& & 1 & 11 & 41 & 101 \\ \hline
CNN & 0.27M & \multicolumn{4}{c}{ 19.59 } \\ \hline
~~~ + Knn & 0.27M + 5K & 6.13 & 6.13 & 6.13 & 6.13 \\ \hline
~~~ + DeepKnn & 0.27M + 5K & 7.59 & 7.59 & 6.13 & 11.07 \\ \hline
Zhang {\em et al.} \cite{Zhang20} & 0.87M & \multicolumn{4}{|c|}{ 89.26 } \\ \hline
~~~ + kNN & 0.87M + 12.8M & 88.28 & 91.69 & 91.7 & 91.61 \\ \hline
~~~ + kNet & 0.87M + 5K & 91.34 & 91.46 & 91.57 & 91.31 \\ \hline
~~~ + fixedkNet & 0.87M + 5K & 91.43 & \textbf{91.81} & 91.42 & 91.09 \\ \hline
\end{tabular}
\end{center}
\caption{SVHN - 80\% uniform noise}
\label{tab:SVHN-80}
\end{table}

\begin{table}
\begin{center}
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
Network & Parameters & \multicolumn{4}{|c|}{ K } \\ \hline
& & 1 & 21 & 41 & 101 \\ \hline
Zhang et al & 0.87M & \multicolumn{4}{|c|}{ 92.59 } \\ \hline
~~~  + kNN & 0.87M + 12.8M & 91.69 & 94.09 & \textbf{94.11} & 93.99 \\ \hline
~~~  + kNet & 0.87M + 5K & 93.3 & 93.51 & 93.78 & 93.4 \\ \hline
~~~  + fixedkNet & 0.87M + 5K & 93.83 & 93.83 & 93.85 & 93.84 \\ \hline
\end{tabular}
\end{center}
\caption{SVHN - 40\% semantic asymmetric noise}
\label{tab:SVHN-80}
\end{table}

\begin{table}
\begin{center}
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
Network & Parameters & \multicolumn{4}{|c|}{ K } \\ \hline
& & 1 & 21 & 51 & 101 \\ \hline
Zhang et al & 0.87M & \multicolumn{4}{|c|}{ 89.76 } \\ \hline
~~~  + kNN & 0.87M + 12.8M & 85.79 & 89.29 & 89.16 & 88.79 \\ \hline
~~~  + Knet & 0.87M + 5K & 88.94 & 89.12 & 89.45 & 88.72 \\ \hline
~~~  + fixed Knet & 0.87M + 5K & \textbf{89.91} & 89.58 & 89.77 & 89.63 \\ \hline
\end{tabular}
\end{center}
\caption{Cifar10 - 40\% semantic asymmetric noise}
\label{tab:SVHN-80}
\end{table}



==> egbib.bib.tex <==

@inproceedings{DroryRAG20,
  author    = {Amnon Drory and
               Oria Ratzon and
               Shai Avidan and
               Raja Giryes},
  title     = {The Resistance to Label Noise in {K-NN} and {DNN} Depends on its Concentration},
  booktitle = {31st British Machine Vision Conference 2020, {BMVC} 2020, Virtual
               Event, UK, September 7-10, 2020},
  publisher = {{BMVA} Press},
  year      = {2020},
  url       = {https://www.bmvc2020-conference.com/assets/papers/0176.pdf},
  timestamp = {Wed, 03 Feb 2021 08:36:16 +0100},
  biburl    = {https://dblp.org/rec/conf/bmvc/DroryRAG20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Arya1998ANNLF,
  title={ANN: library for approximate nearest neighbor searching},
  author={S. Arya and D. Mount},
  year={1998}
}

@inproceedings{LSH,
author = {Indyk, Piotr and Motwani, Rajeev},
title = {Approximate Nearest Neighbors: Towards Removing the Curse of Dimensionality},
year = {1998},
isbn = {0897919629},
publisher = {Association for Computing Machinery},
booktitle = {Proceedings of the Thirtieth Annual ACM Symposium on Theory of Computing},
pages = {604–613},
numpages = {10},
series = {STOC '98}
}

@inproceedings{Zhang20,
title	= {Distilling Effective Supervision from Severe Label Noise},
author	= {Zizhao Zhang and Han Zhang and Sercan Arik and Honglak Lee and Tomas Pfister},
year	= {2020},
URL	= {https://arxiv.org/pdf/1910.00701.pdf},
booktitle	= {CVPR}
}

@article{DBLP:journals/corr/abs-2007-03212,
  author    = {Doyup Lee and
               Yeongjae Cheon},
  title     = {Soft Labeling Affects Out-of-Distribution Detection of Deep Neural
               Networks},
  journal   = {CoRR},
  volume    = {abs/2007.03212},
  year      = {2020},
  url       = {https://arxiv.org/abs/2007.03212},
  archivePrefix = {arXiv},
  eprint    = {2007.03212},
  timestamp = {Mon, 20 Jul 2020 14:20:39 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2007-03212.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{SukhbaatarF14,
  author    = {Sainbayar Sukhbaatar and
               Rob Fergus},
  editor    = {Yoshua Bengio and
               Yann LeCun},
  title     = {Learning from Noisy Labels with Deep Neural Networks},
  booktitle = {3rd International Conference on Learning Representations, {ICLR} 2015,
               San Diego, CA, USA, May 7-9, 2015, Workshop Track Proceedings},
  year      = {2015},
  url       = {http://arxiv.org/abs/1406.2080},
  timestamp = {Wed, 17 Jul 2019 10:40:54 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/SukhbaatarF14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{abs-2007-08199,
  author    = {Hwanjun Song and
               Minseok Kim and
               Dongmin Park and
               Jae{-}Gil Lee},
  title     = {Learning from Noisy Labels with Deep Neural Networks: {A} Survey},
  journal   = {CoRR},
  volume    = {abs/2007.08199},
  year      = {2020},
  url       = {https://arxiv.org/abs/2007.08199},
  archivePrefix = {arXiv},
  eprint    = {2007.08199},
  timestamp = {Wed, 22 Jul 2020 12:09:15 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2007-08199.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/cvpr/XiaoXYHW15,
  author    = {Tong Xiao and
               Tian Xia and
               Yi Yang and
               Chang Huang and
               Xiaogang Wang},
  title     = {Learning from massive noisy labeled data for image classification},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               2015, Boston, MA, USA, June 7-12, 2015},
  pages     = {2691--2699},
  publisher = {{IEEE} Computer Society},
  year      = {2015},
  url       = {https://doi.org/10.1109/CVPR.2015.7298885},
  doi       = {10.1109/CVPR.2015.7298885},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/XiaoXYHW15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/iclr/KhetanLA18,
  author    = {Ashish Khetan and
               Zachary C. Lipton and
               Animashree Anandkumar},
  title     = {Learning From Noisy Singly-labeled Data},
  booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
               Vancouver, BC, Canada, April 30 - May 3, 2018, Conference Track Proceedings},
  year      = {2018},
  url       = {https://openreview.net/forum?id=H1sUHgb0Z},
  timestamp = {Thu, 25 Jul 2019 14:25:41 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/KhetanLA18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/GaoNZ16,
  author    = {Wei Gao and
               Xin{-}Yi Niu and
               Zhi{-}Hua Zhou},
  title     = {On the Consistency of Exact and Approximate Nearest Neighbor with
               Noisy Data},
  journal   = {CoRR},
  volume    = {abs/1607.07526},
  year      = {2016},
  url       = {http://arxiv.org/abs/1607.07526},
  archivePrefix = {arXiv},
  eprint    = {1607.07526},
  timestamp = {Mon, 13 Aug 2018 16:46:37 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/GaoNZ16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/corr/abs-1803-04765,
  author    = {Nicolas Papernot and
               Patrick D. McDaniel},
  title     = {Deep k-Nearest Neighbors: Towards Confident, Interpretable and Robust
               Deep Learning},
  journal   = {CoRR},
  volume    = {abs/1803.04765},
  year      = {2018},
  url       = {http://arxiv.org/abs/1803.04765},
  archivePrefix = {arXiv},
  eprint    = {1803.04765},
  timestamp = {Mon, 13 Aug 2018 16:48:06 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1803-04765.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/icitcs/AgrawalR15,
  author    = {Rashmi Agrawal and
               Babu Ram},
  title     = {A Modified K-Nearest Neighbor Algorithm to Handle Uncertain Data},
  booktitle = {5th International Conference on {IT} Convergence and Security, {ICITCS}
               2015, Kuala Lumpur, Malaysia, August 24-27, 2015},
  pages     = {1--4},
  publisher = {{IEEE} Computer Society},
  year      = {2015},
  url       = {https://doi.org/10.1109/ICITCS.2015.7292920},
  doi       = {10.1109/ICITCS.2015.7292920},
  timestamp = {Sat, 19 Oct 2019 20:22:20 +0200},
  biburl    = {https://dblp.org/rec/conf/icitcs/AgrawalR15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/nips/HendrycksMWG18,
  author    = {Dan Hendrycks and
               Mantas Mazeika and
               Duncan Wilson and
               Kevin Gimpel},
  editor    = {Samy Bengio and
               Hanna M. Wallach and
               Hugo Larochelle and
               Kristen Grauman and
               Nicol{\`{o}} Cesa{-}Bianchi and
               Roman Garnett},
  title     = {Using Trusted Data to Train Deep Networks on Labels Corrupted by Severe
               Noise},
  booktitle = {Advances in Neural Information Processing Systems 31: Annual Conference
               on Neural Information Processing Systems 2018, NeurIPS 2018, December
               3-8, 2018, Montr{\'{e}}al, Canada},
  pages     = {10477--10486},
  year      = {2018},
  url       = {https://proceedings.neurips.cc/paper/2018/hash/ad554d8c3b06d6b97ee76a2448bd7913-Abstract.html},
  timestamp = {Thu, 21 Jan 2021 15:15:21 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/HendrycksMWG18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/aaai/GhoshKS17,
  author    = {Aritra Ghosh and
               Himanshu Kumar and
               P. S. Sastry},
  editor    = {Satinder P. Singh and
               Shaul Markovitch},
  title     = {Robust Loss Functions under Label Noise for Deep Neural Networks},
  booktitle = {Proceedings of the Thirty-First {AAAI} Conference on Artificial Intelligence,
               February 4-9, 2017, San Francisco, California, {USA}},
  pages     = {1919--1925},
  publisher = {{AAAI} Press},
  year      = {2017},
  url       = {http://aaai.org/ocs/index.php/AAAI/AAAI17/paper/view/14759},
  timestamp = {Wed, 10 Feb 2021 08:43:31 +0100},
  biburl    = {https://dblp.org/rec/conf/aaai/GhoshKS17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/nips/ZhangS18,
  author    = {Zhilu Zhang and
               Mert R. Sabuncu},
  editor    = {Samy Bengio and
               Hanna M. Wallach and
               Hugo Larochelle and
               Kristen Grauman and
               Nicol{\`{o}} Cesa{-}Bianchi and
               Roman Garnett},
  title     = {Generalized Cross Entropy Loss for Training Deep Neural Networks with
               Noisy Labels},
  booktitle = {Advances in Neural Information Processing Systems 31: Annual Conference
               on Neural Information Processing Systems 2018, NeurIPS 2018, December
               3-8, 2018, Montr{\'{e}}al, Canada},
  pages     = {8792--8802},
  year      = {2018},
  url       = {https://proceedings.neurips.cc/paper/2018/hash/f2925f97bc13ad2852a7a551802feea0-Abstract.html},
  timestamp = {Thu, 21 Jan 2021 15:15:21 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/ZhangS18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/iccv/0001MCLY019,
  author    = {Yisen Wang and
               Xingjun Ma and
               Zaiyi Chen and
               Yuan Luo and
               Jinfeng Yi and
               James Bailey},
  title     = {Symmetric Cross Entropy for Robust Learning With Noisy Labels},
  booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
               2019, Seoul, Korea (South), October 27 - November 2, 2019},
  pages     = {322--330},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/ICCV.2019.00041},
  doi       = {10.1109/ICCV.2019.00041},
  timestamp = {Thu, 05 Mar 2020 13:43:22 +0100},
  biburl    = {https://dblp.org/rec/conf/iccv/0001MCLY019.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/iclr/LyuT20,
  author    = {Yueming Lyu and
               Ivor W. Tsang},
  title     = {Curriculum Loss: Robust Learning and Generalization against Label
               Corruption},
  booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
               Addis Ababa, Ethiopia, April 26-30, 2020},
  year      = {2020},
  timestamp = {Thu, 07 May 2020 17:11:47 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/LyuT20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/air/VilaltaD02,
  author    = {Ricardo Vilalta and
               Youssef Drissi},
  title     = {A Perspective View and Survey of Meta-Learning},
  journal   = {Artif. Intell. Rev.},
  volume    = {18},
  number    = {2},
  pages     = {77--95},
  year      = {2002},
  url       = {https://doi.org/10.1023/A:1019956318069},
  doi       = {10.1023/A:1019956318069},
  timestamp = {Wed, 17 May 2017 14:25:43 +0200},
  biburl    = {https://dblp.org/rec/journals/air/VilaltaD02.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/cvpr/HeZ0ZXL19,
  author    = {Tong He and
               Zhi Zhang and
               Hang Zhang and
               Zhongyue Zhang and
               Junyuan Xie and
               Mu Li},
  title     = {Bag of Tricks for Image Classification with Convolutional Neural Networks},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               2019, Long Beach, CA, USA, June 16-20, 2019},
  pages     = {558--567},
  publisher = {Computer Vision Foundation / {IEEE}},
  year      = {2019},
  url       = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/He\_Bag\_of\_Tricks\_for\_Image\_Classification\_with\_Convolutional\_Neural\_Networks\_CVPR\_2019\_paper.html},
  doi       = {10.1109/CVPR.2019.00065},
  timestamp = {Tue, 22 Sep 2020 07:46:20 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/HeZ0ZXL19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/nips/MullerKH19,
  author    = {Rafael M{\"{u}}ller and
               Simon Kornblith and
               Geoffrey E. Hinton},
  editor    = {Hanna M. Wallach and
               Hugo Larochelle and
               Alina Beygelzimer and
               Florence d'Alch{\'{e}}{-}Buc and
               Emily B. Fox and
               Roman Garnett},
  title     = {When does label smoothing help?},
  booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
               on Neural Information Processing Systems 2019, NeurIPS 2019, December
               8-14, 2019, Vancouver, BC, Canada},
  pages     = {4696--4705},
  year      = {2019},
  url       = {https://proceedings.neurips.cc/paper/2019/hash/f1748d6b0fd9d439f71450117eba2725-Abstract.html},
  timestamp = {Thu, 21 Jan 2021 15:15:19 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/MullerKH19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-1909-11723,
  author    = {Li Yuan and
               Francis E. H. Tay and
               Guilin Li and
               Tao Wang and
               Jiashi Feng},
  title     = {Revisit Knowledge Distillation: a Teacher-free Framework},
  journal   = {CoRR},
  volume    = {abs/1909.11723},
  year      = {2019},
  url       = {http://arxiv.org/abs/1909.11723},
  archivePrefix = {arXiv},
  eprint    = {1909.11723},
  timestamp = {Thu, 19 Nov 2020 20:36:33 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1909-11723.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/icml/LukasikBMK20,
  author    = {Michal Lukasik and
               Srinadh Bhojanapalli and
               Aditya Krishna Menon and
               Sanjiv Kumar},
  title     = {Does label smoothing mitigate label noise?},
  booktitle = {Proceedings of the 37th International Conference on Machine Learning,
               {ICML} 2020, 13-18 July 2020, Virtual Event},
  series    = {Proceedings of Machine Learning Research},
  volume    = {119},
  pages     = {6448--6458},
  publisher = {{PMLR}},
  year      = {2020},
  url       = {http://proceedings.mlr.press/v119/lukasik20a.html},
  timestamp = {Tue, 15 Dec 2020 17:40:19 +0100},
  biburl    = {https://dblp.org/rec/conf/icml/LukasikBMK20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/cvpr/PatriniRMNQ17,
  author    = {Giorgio Patrini and
               Alessandro Rozza and
               Aditya Krishna Menon and
               Richard Nock and
               Lizhen Qu},
  title     = {Making Deep Neural Networks Robust to Label Noise: {A} Loss Correction
               Approach},
  booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
  pages     = {2233--2241},
  publisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {https://doi.org/10.1109/CVPR.2017.240},
  doi       = {10.1109/CVPR.2017.240},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/PatriniRMNQ17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/corr/abs-1805-06822,
  author    = {Gilad Cohen and
               Guillermo Sapiro and
               Raja Giryes},
  title     = {{DNN} or k-NN: That is the Generalize vs. Memorize Question},
  journal   = {CoRR},
  volume    = {abs/1805.06822},
  year      = {2018},
  url       = {http://arxiv.org/abs/1805.06822},
  archivePrefix = {arXiv},
  eprint    = {1805.06822},
  timestamp = {Mon, 13 Aug 2018 16:48:42 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1805-06822.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/icml/WangJC18,
  author    = {Yizhen Wang and
               Somesh Jha and
               Kamalika Chaudhuri},
  editor    = {Jennifer G. Dy and
               Andreas Krause},
  title     = {Analyzing the Robustness of Nearest Neighbors to Adversarial Examples},
  booktitle = {Proceedings of the 35th International Conference on Machine Learning,
               {ICML} 2018, Stockholmsm{\"{a}}ssan, Stockholm, Sweden, July
               10-15, 2018},
  series    = {Proceedings of Machine Learning Research},
  volume    = {80},
  pages     = {5120--5129},
  publisher = {{PMLR}},
  year      = {2018},
  url       = {http://proceedings.mlr.press/v80/wang18c.html},
  timestamp = {Wed, 03 Apr 2019 18:17:30 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/WangJC18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/iclr/ZhangBHRV17,
  author    = {Chiyuan Zhang and
               Samy Bengio and
               Moritz Hardt and
               Benjamin Recht and
               Oriol Vinyals},
  title     = {Understanding deep learning requires rethinking generalization},
  booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
               Toulon, France, April 24-26, 2017, Conference Track Proceedings},
  year      = {2017},
  url       = {https://openreview.net/forum?id=Sy8gdB9xx},
  timestamp = {Thu, 04 Apr 2019 13:20:08 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/ZhangBHRV17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/iclr/GoldbergerB17,
  author    = {Jacob Goldberger and
               Ehud Ben{-}Reuven},
  title     = {Training deep neural-networks using a noise adaptation layer},
  booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
               Toulon, France, April 24-26, 2017, Conference Track Proceedings},
  year      = {2017},
  url       = {https://openreview.net/forum?id=H12GRgcxg},
  timestamp = {Thu, 25 Jul 2019 14:25:42 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/GoldbergerB17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/corr/abs-2009-14757,
  author    = {Zhenzhen Wang and
               Chunyan Xu and
               Yap{-}Peng Tan and
               Junsong Yuan},
  title     = {Attention-Aware Noisy Label Learning for Image Classification},
  journal   = {CoRR},
  volume    = {abs/2009.14757},
  year      = {2020},
  url       = {https://arxiv.org/abs/2009.14757},
  archivePrefix = {arXiv},
  eprint    = {2009.14757},
  timestamp = {Wed, 07 Oct 2020 15:59:26 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2009-14757.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/ml/WilsonM00,
  author    = {D. Randall Wilson and
               Tony R. Martinez},
  title     = {Reduction Techniques for Instance-Based Learning Algorithms},
  journal   = {Mach. Learn.},
  volume    = {38},
  number    = {3},
  pages     = {257--286},
  year      = {2000},
  url       = {https://doi.org/10.1023/A:1007626913721},
  doi       = {10.1023/A:1007626913721},
  timestamp = {Mon, 02 Mar 2020 16:30:00 +0100},
  biburl    = {https://dblp.org/rec/journals/ml/WilsonM00.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/corr/abs-1708-04321,
  author    = {V. B. Surya Prasath and
               Haneen Arafat Abu Alfeilat and
               Omar Lasassmeh and
               Ahmad B. A. Hassanat},
  title     = {Distance and Similarity Measures Effect on the Performance of K-Nearest
               Neighbor Classifier - {A} Review},
  journal   = {CoRR},
  volume    = {abs/1708.04321},
  year      = {2017},
  url       = {http://arxiv.org/abs/1708.04321},
  archivePrefix = {arXiv},
  eprint    = {1708.04321},
  timestamp = {Sat, 23 Jan 2021 01:19:33 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1708-04321.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/icml/ShenS19,
  author    = {Yanyao Shen and
               Sujay Sanghavi},
  editor    = {Kamalika Chaudhuri and
               Ruslan Salakhutdinov},
  title     = {Learning with Bad Training Data via Iterative Trimmed Loss Minimization},
  booktitle = {Proceedings of the 36th International Conference on Machine Learning,
               {ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
  series    = {Proceedings of Machine Learning Research},
  volume    = {97},
  pages     = {5739--5748},
  publisher = {{PMLR}},
  year      = {2019},
  url       = {http://proceedings.mlr.press/v97/shen19e.html},
  timestamp = {Tue, 11 Jun 2019 15:37:38 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/ShenS19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/jaciii/JeatrakulWF10,
  author    = {Piyasak Jeatrakul and
               Kok Wai Wong and
               Chun Che Fung},
  title     = {Data Cleaning for Classification Using Misclassification Analysis},
  journal   = {J. Adv. Comput. Intell. Intell. Informatics},
  volume    = {14},
  number    = {3},
  pages     = {297--302},
  year      = {2010},
  url       = {https://doi.org/10.20965/jaciii.2010.p0297},
  doi       = {10.20965/jaciii.2010.p0297},
  timestamp = {Tue, 16 Feb 2021 08:58:27 +0100},
  biburl    = {https://dblp.org/rec/journals/jaciii/JeatrakulWF10.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/cvpr/WangLMBZSX18,
  author    = {Yisen Wang and
               Weiyang Liu and
               Xingjun Ma and
               James Bailey and
               Hongyuan Zha and
               Le Song and
               Shu{-}Tao Xia},
  title     = {Iterative Learning With Open-Set Noisy Labels},
  booktitle = {2018 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2018, Salt Lake City, UT, USA, June 18-22, 2018},
  pages     = {8688--8696},
  publisher = {{IEEE} Computer Society},
  year      = {2018},
  url       = {http://openaccess.thecvf.com/content\_cvpr\_2018/html/Wang\_Iterative\_Learning\_With\_CVPR\_2018\_paper.html},
  doi       = {10.1109/CVPR.2018.00906},
  timestamp = {Sun, 27 Oct 2019 17:57:12 +0100},
  biburl    = {https://dblp.org/rec/conf/cvpr/WangLMBZSX18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/jair/BrodleyF99,
  author    = {Carla E. Brodley and
               Mark A. Friedl},
  title     = {Identifying Mislabeled Training Data},
  journal   = {J. Artif. Intell. Res.},
  volume    = {11},
  pages     = {131--167},
  year      = {1999},
  url       = {https://doi.org/10.1613/jair.606},
  doi       = {10.1613/jair.606},
  timestamp = {Mon, 21 Jan 2019 15:01:18 +0100},
  biburl    = {https://dblp.org/rec/journals/jair/BrodleyF99.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/icml/BahriJG20,
  author    = {Dara Bahri and
               Heinrich Jiang and
               Maya R. Gupta},
  title     = {Deep k-NN for Noisy Labels},
  booktitle = {Proceedings of the 37th International Conference on Machine Learning,
               {ICML} 2020, 13-18 July 2020, Virtual Event},
  series    = {Proceedings of Machine Learning Research},
  volume    = {119},
  pages     = {540--550},
  publisher = {{PMLR}},
  year      = {2020},
  url       = {http://proceedings.mlr.press/v119/bahri20a.html},
  timestamp = {Tue, 15 Dec 2020 17:40:18 +0100},
  biburl    = {https://dblp.org/rec/conf/icml/BahriJG20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/icml/ThulasidasanBBC19,
  author    = {Sunil Thulasidasan and
               Tanmoy Bhattacharya and
               Jeff A. Bilmes and
               Gopinath Chennupati and
               Jamal Mohd{-}Yusof},
  editor    = {Kamalika Chaudhuri and
               Ruslan Salakhutdinov},
  title     = {Combating Label Noise in Deep Learning using Abstention},
  booktitle = {Proceedings of the 36th International Conference on Machine Learning,
               {ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
  series    = {Proceedings of Machine Learning Research},
  volume    = {97},
  pages     = {6234--6243},
  publisher = {{PMLR}},
  year      = {2019},
  url       = {http://proceedings.mlr.press/v97/thulasidasan19a.html},
  timestamp = {Tue, 11 Jun 2019 15:37:38 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/ThulasidasanBBC19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/ijon/TomasevB15,
  author    = {Nenad Tomasev and
               Krisztian Buza},
  title     = {Hubness-aware kNN classification of high-dimensional data in presence
               of label noise},
  journal   = {Neurocomputing},
  volume    = {160},
  pages     = {157--172},
  year      = {2015},
  url       = {https://doi.org/10.1016/j.neucom.2014.10.084},
  doi       = {10.1016/j.neucom.2014.10.084},
  timestamp = {Sun, 02 Jun 2019 20:50:26 +0200},
  biburl    = {https://dblp.org/rec/journals/ijon/TomasevB15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/cvpr/SzegedyVISW16,
  author    = {Christian Szegedy and
               Vincent Vanhoucke and
               Sergey Ioffe and
               Jonathon Shlens and
               Zbigniew Wojna},
  title     = {Rethinking the Inception Architecture for Computer Vision},
  booktitle = {2016 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2016, Las Vegas, NV, USA, June 27-30, 2016},
  pages     = {2818--2826},
  publisher = {{IEEE} Computer Society},
  year      = {2016},
  url       = {https://doi.org/10.1109/CVPR.2016.308},
  doi       = {10.1109/CVPR.2016.308},
  timestamp = {Sun, 25 Oct 2020 23:02:11 +0100},
  biburl    = {https://dblp.org/rec/conf/cvpr/SzegedyVISW16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-2009-08233,
  author    = {Chaohao Fu and
               Hongbin Chen and
               Na Ruan and
               Weijia Jia},
  title     = {Label Smoothing and Adversarial Robustness},
  journal   = {CoRR},
  volume    = {abs/2009.08233},
  year      = {2020},
  url       = {https://arxiv.org/abs/2009.08233},
  archivePrefix = {arXiv},
  eprint    = {2009.08233},
  timestamp = {Wed, 25 Nov 2020 13:17:36 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2009-08233.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/corr/abs-2007-05836,
  author    = {G{\"{o}}rkem Algan and
               Ilkay Ulusoy},
  title     = {Meta Soft Label Generation for Noisy Labels},
  journal   = {CoRR},
  volume    = {abs/2007.05836},
  year      = {2020},
  url       = {https://arxiv.org/abs/2007.05836},
  archivePrefix = {arXiv},
  eprint    = {2007.05836},
  timestamp = {Mon, 20 Jul 2020 14:20:39 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2007-05836.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/iccbr/OkamotoS95,
  author    = {Seishi Okamoto and
               Ken Satoh},
  editor    = {Manuela M. Veloso and
               Agnar Aamodt},
  title     = {An Average-Case Analysis of k-Nearest Neighbor Classifier},
  booktitle = {Case-Based Reasoning Research and Development, First International
               Conference, ICCBR-95, Sesimbra, Portugal, October 23-26, 1995, Proceedings},
  series    = {Lecture Notes in Computer Science},
  volume    = {1010},
  pages     = {253--264},
  publisher = {Springer},
  year      = {1995},
  url       = {https://doi.org/10.1007/3-540-60598-3\_23},
  doi       = {10.1007/3-540-60598-3\_23},
  timestamp = {Fri, 27 Dec 2019 21:24:11 +0100},
  biburl    = {https://dblp.org/rec/conf/iccbr/OkamotoS95.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{tsne,
  author = {van der Maaten, Laurens and Hinton, Geoffrey E.},
  biburl = {https://www.bibsonomy.org/bibtex/25fde64f4b6ca95060a329b980a54013f/saos},
  interhash = {d3658497eff9fea21e66bb43320a822a},
  intrahash = {5fde64f4b6ca95060a329b980a54013f},
  journal = {Journal of Machine Learning Research},
  keywords = {dimensionality_reduction visualization},
  pages = {2579-2605},
  timestamp = {2015-04-29T17:59:14.000+0200},
  title = {Visualizing High-Dimensional Data Using t-SNE},
  volume = 9,
  year = 2008
}

